CREST: A Joint Framework for Rationalization and Counterfactual Text Generation

Selective rationales and counterfactual examples have emerged as two effective, complementary classes of interpretability methods for analyzing and training NLP models. However, prior work has not explored how these methods can be integrated to combine their complementary advantages. We overcome this limitation by introducing CREST (ContRastive Edits with Sparse raTionalization), a joint framework for selective rationalization and counterfactual text generation, and show that this framework leads to improvements in counterfactual quality, model robustness, and interpretability. First, CREST generates valid counterfactuals that are more natural than those produced by previous methods, and subsequently can be used for data augmentation at scale, reducing the need for human-generated examples. Second, we introduce a new loss function that leverages CREST counterfactuals to regularize selective rationales and show that this regularization improves both model robustness and rationale quality, compared to methods that do not leverage CREST counterfactuals. Our results demonstrate that CREST successfully bridges the gap between selective rationales and counterfactual examples, addressing the limitations of existing methods and providing a more comprehensive view of a model's predictions.

==> tables/results_iid_con_ood_backup_19jan_imdb.tex <==
\definecolor{ccon}{HTML}{fee9d4}
\definecolor{cood}{HTML}{d8f0d3}
\definecolor{cid}{HTML}{dae8f5}

\begin{table*}[!htb]
    \small
    \centering
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l@{}rccccccc}
        \toprule
        \bf Setup & \bf Data size & \bf \cellcolor{cid}{IMDB} & \bf \cellcolor{ccon}{rIMDB} & \bf \cellcolor{ccon}{cIMDB} & \bf \cellcolor{cood}{RotTom} & \bf \cellcolor{cood}{SST-2} & \bf \cellcolor{cood}{Amazon} & \bf \cellcolor{cood}{Yelp}\\

        \midrule
        $F$ & 100\%                   & 91.1 \scriptsize{$\pm$ 0.3} & 91.4 \scriptsize{$\pm$ 0.8} & 88.5 \scriptsize{$\pm$ 0.9} & 76.5 \scriptsize{$\pm$ 1.6}  & 79.8 \scriptsize{$\pm$ 1.6}  & 86.0 \scriptsize{$\pm$ 0.7}  & 88.5 \scriptsize{$\pm$ 0.7} \\
        
        $F + C_H$ & +8\%      & 90.9 \scriptsize{$\pm$ 0.5} & 92.9 \scriptsize{$\pm$ 0.9} & 90.4 \scriptsize{$\pm$ 1.6} & 76.6 \scriptsize{$\pm$ 1.5}  & 80.7 \scriptsize{$\pm$ 1.3}  & 86.3 \scriptsize{$\pm$ 1.0}  & 89.1 \scriptsize{$\pm$ 1.2} \\

        \cdashlinelr{1-9}
        $F + C_{S,V}$ & +1\%  & 90.8 \scriptsize{$\pm$ 0.2} & 91.5 \scriptsize{$\pm$ 0.5} & 89.1 \scriptsize{$\pm$ 0.6} & 77.2 \scriptsize{$\pm$ 1.1}  & 80.5 \scriptsize{$\pm$ 0.5}  & 86.1 \scriptsize{$\pm$ 0.2}  & 88.8 \scriptsize{$\pm$ 0.3}  \\
        $F + C_{S,V}$ & +2\%  & 91.1 \scriptsize{$\pm$ 0.4} & 91.3 \scriptsize{$\pm$ 1.6} & 88.6 \scriptsize{$\pm$ 1.2} & 76.2 \scriptsize{$\pm$ 1.2}  & 80.8 \scriptsize{$\pm$ 0.8}  & 86.7 \scriptsize{$\pm$ 0.5}  & 89.6 \scriptsize{$\pm$ 0.5}  \\
        $F + C_{S,V}$ & +4\%  & 91.1 \scriptsize{$\pm$ 0.1} & 91.6 \scriptsize{$\pm$ 1.2} & 89.3 \scriptsize{$\pm$ 0.9} & 77.7 \scriptsize{$\pm$ 0.8}  & 80.8 \scriptsize{$\pm$ 0.7}  & 87.0 \scriptsize{$\pm$ 0.6}  & 89.8 \scriptsize{$\pm$ 0.6}  \\
        $F + C_{S,V}$ & +8\%  & 90.7 \scriptsize{$\pm$ 0.6} & 91.5 \scriptsize{$\pm$ 1.2} & 88.8 \scriptsize{$\pm$ 1.1} & 76.6 \scriptsize{$\pm$ 2.2}  & 80.2 \scriptsize{$\pm$ 1.7}  & 86.1 \scriptsize{$\pm$ 0.9}  & 88.2 \scriptsize{$\pm$ 1.0}  \\

        \cdashlinelr{1-9}
        $F + C_{S,V}$ & +85\%  & 90.0 \scriptsize{$\pm$ 0.4} & 92.1 \scriptsize{$\pm$ 0.8} & 89.7 \scriptsize{$\pm$ 0.5} & 75.8 \scriptsize{$\pm$ 0.4}  & 79.2 \scriptsize{$\pm$ 1.2}  & 85.9 \scriptsize{$\pm$ 0.7}  & 88.0 \scriptsize{$\pm$ 1.1} \\
        $F + C_{S,V}$ (new) & +85\%  & 91.0 \scriptsize{$\pm$ 0.2} & 91.2 \scriptsize{$\pm$ 1.0} & 89.3 \scriptsize{$\pm$ 0.8} & 76.8 \scriptsize{$\pm$ 0.9} & 79.3 \scriptsize{$\pm$ 0.3} & 85.2 \scriptsize{$\pm$ 0.9} & 88.0 \scriptsize{$\pm$ 1.0}  \\
        
        $F + C_{S}$ & +100\%    & 89.7 \scriptsize{$\pm$ 0.6} & 92.6 \scriptsize{$\pm$ 0.7} & 89.8 \scriptsize{$\pm$ 0.8} & 73.1 \scriptsize{$\pm$ 2.8}  & 75.4 \scriptsize{$\pm$ 3.3}  & 84.2 \scriptsize{$\pm$ 2.0}  & 87.3 \scriptsize{$\pm$ 1.7} \\
        $F + C_{S}$ (new) & +100\%    & 90.8 \scriptsize{$\pm$ 0.2} & 91.6 \scriptsize{$\pm$ 1.3} & 89.2 \scriptsize{$\pm$ 0.4} & 76.7 \scriptsize{$\pm$ 1.0} & 80.6 \scriptsize{$\pm$ 0.6} & 86.4 \scriptsize{$\pm$ 0.6} & 89.1 \scriptsize{$\pm$ 0.5} \\
        
        \cdashlinelr{1-9}
        \multicolumn{2}{l}{\textit{With agreement regularization:}} \\
        $F\ \&\ C_{S, V}$ & 85\%     & 90.7 \scriptsize{$\pm$ 0.1} & 93.1 \scriptsize{$\pm$ 0.5} & 90.3 \scriptsize{$\pm$ 0.4} & 75.0 \scriptsize{$\pm$ 2.2}  & 78.1 \scriptsize{$\pm$ 1.7}  & 86.2 \scriptsize{$\pm$ 0.6}  & 88.7 \scriptsize{$\pm$ 0.7} \\
        $F\ \&\ C_{S, V}$ (new) & 85\%     & 90.7 \scriptsize{$\pm$ 0.5} & 92.2 \scriptsize{$\pm$ 0.7} & 88.9 \scriptsize{$\pm$ 1.0} & 76.3 \scriptsize{$\pm$ 1.4} & 80.2 \scriptsize{$\pm$ 1.3} & 86.3 \scriptsize{$\pm$ 0.7} & 88.9 \scriptsize{$\pm$ 0.7}  \\
        
        $F\ \&\ C_{S}$ & 100\%       & 90.1 \scriptsize{$\pm$ 0.2} & 93.2 \scriptsize{$\pm$ 0.5} & 90.7 \scriptsize{$\pm$ 0.4} & 72.4 \scriptsize{$\pm$ 2.1}  & 74.6 \scriptsize{$\pm$ 2.3}  & 84.0 \scriptsize{$\pm$ 0.6}  & 87.8 \scriptsize{$\pm$ 0.7} \\
        $F\ \&\ C_{S}$ (new) & 100\%      & 91.2 \scriptsize{$\pm$ 0.5} & 92.8 \scriptsize{$\pm$ 0.5} & 89.7 \scriptsize{$\pm$ 1.1} & 77.3 \scriptsize{$\pm$ 2.3} & 81.1 \scriptsize{$\pm$ 2.4} & 86.8 \scriptsize{$\pm$ 0.8} & 89.3 \scriptsize{$\pm$ 0.7}  \\
        
        \bottomrule
    \end{tabular}
    \caption{
    Accuracy of SPECTRA trained on IMDB with different data augmentation setups on \colorbox{cid}{in-domain}, \colorbox{ccon}{contrast}, and \colorbox{cood}{out-of-domain} datasets: we compare a standard SPECTRA trained on factual examples ($F$) with other SPECTRA models trained on augmentated data from human-crafted counterfactuals ($F + C_H$) and synthetic counterfactuals generated by CREST ($F + C_S$), which we additionally post-process to drop invalid examples ($F + C_{S,V}$). We present the mean and standard deviation across five random seeds.}
    \label{tab:results_rationalizers_in_domain}
\end{table*}


\begin{table*}[!htb]
    \small
    \centering
    \begin{tabular}{l c@{\tquad}c@{\tquad}c}
        \toprule
        \bf Setup & \bf Plausibility & \bf F. sim. & \bf C. sim. \\
        \midrule
        $F$                           & 0.6733  \scriptsize{$\pm$ 0.02} & 91.70 \scriptsize{$\pm$ 0.92} & 81.18 \scriptsize{$\pm$ 2.79} \\
        $F + C_H$                     & 0.6718  \scriptsize{$\pm$ 0.04} & 91.44 \scriptsize{$\pm$ 1.46} & 80.53 \scriptsize{$\pm$ 4.17} \\
        $F + C_S$                 & 0.6758  \scriptsize{$\pm$ 0.02} & 91.11 \scriptsize{$\pm$ 1.04} & 88.58 \scriptsize{$\pm$ 2.52} \\
        
        $F + C_S$ (new)                 & 0.6938  \scriptsize{$\pm$ 0.01} & 91.68 \scriptsize{$\pm$ 0.59} & 84.54 \scriptsize{$\pm$ 1.09} \\
        
        \cdashlinelr{1-4}
        \multicolumn{3}{l}{\textit{With agreement regularization:}} \\
        $F\ \&\ C_S$ & 0.7040  \scriptsize{$\pm$ 0.01} & 91.84 \scriptsize{$\pm$ 0.76} & 88.78 \scriptsize{$\pm$ 1.14} \\
        
        $F\ \&\ C_S$ (new) & 0.6904  \scriptsize{$\pm$ 0.02} & 91.93 \scriptsize{$\pm$ 0.83} & 86.43 \scriptsize{$\pm$ 1.56} \\
        \bottomrule
    \end{tabular}
    \caption{Interpretability analysis. Plausibility represents matching with human rationales in terms of AUC, whereas F. sim. and C. sim. represent forward and counterfactual simulability, respectively.}
\end{table*}


==> tables/results_iid_con_ood_backup_19jan_snli.tex <==
\begin{table*}[t]
    \small
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l@{}rcccccccc}
        \toprule
        \textbf{Setup} & \bf Data Size & \cellcolor{cid}{SNLI} & \cellcolor{cid}{HNLI-e} & \cellcolor{cid}{HNLI-h} & \cellcolor{ccon}{rSNLI} & \cellcolor{ccon}{break} & \cellcolor{cood}{MNLI-m} & \cellcolor{cood}{MNLI-mm} & \cellcolor{cood}{ANLI}  \\

        \midrule
        $F$ & 100\%                   & \bf 84.4 \scriptsize{$\pm$ 0.3} & \bf 90.4 \scriptsize{$\pm$ 1.5} & 70.5 \scriptsize{$\pm$ 3.1}  & 67.8 \scriptsize{$\pm$ 1.1} & 68.4 \scriptsize{$\pm$ 0.9} & \bf 62.5 \scriptsize{$\pm$ 0.6}  & 64.2 \scriptsize{$\pm$ 0.7}  & 31.7 \scriptsize{$\pm$ 1.0}      \\
        
        $F + C_H$ & +1.2\%      & 84.1 \scriptsize{$\pm$ 0.2} & 89.8 \scriptsize{$\pm$ 0.8} & 71.8 \scriptsize{$\pm$ 2.3}  & 67.8 \scriptsize{$\pm$ 0.4} & 67.8 \scriptsize{$\pm$ 1.9} & \bf 62.5 \scriptsize{$\pm$ 0.5}  & 64.2 \scriptsize{$\pm$ 0.7}  & 31.4 \scriptsize{$\pm$ 0.8}      \\

        \cdashlinelr{1-10}
        
        $F + C_{S,V}$ & +0.25\%   & 84.2 \scriptsize{$\pm$ 0.3} & 89.4 \scriptsize{$\pm$ 2.0} & 70.5 \scriptsize{$\pm$ 2.6}  & 67.7 \scriptsize{$\pm$ 0.7} & 67.2 \scriptsize{$\pm$ 2.7} & 62.2 \scriptsize{$\pm$ 0.2}  & 64.2 \scriptsize{$\pm$ 0.3}  & 31.0 \scriptsize{$\pm$ 0.6}      \\
        $F + C_{S,V}$ & +0.5\%   & 84.3 \scriptsize{$\pm$ 0.3} & 89.6 \scriptsize{$\pm$ 1.8} & 70.1 \scriptsize{$\pm$ 1.3}  & \bf 68.2 \scriptsize{$\pm$ 0.4} & 68.4 \scriptsize{$\pm$ 3.0} & 62.4 \scriptsize{$\pm$ 0.6}  & 63.9 \scriptsize{$\pm$ 0.7}  & 31.2 \scriptsize{$\pm$ 1.5}      \\
        $F + C_{S,V}$ & +1.0\%    & 84.2 \scriptsize{$\pm$ 0.4} & 88.4 \scriptsize{$\pm$ 1.6} & 69.6 \scriptsize{$\pm$ 1.7}  & 67.4 \scriptsize{$\pm$ 0.3} & 66.9 \scriptsize{$\pm$ 2.0} & 61.8 \scriptsize{$\pm$ 0.4}  & 63.9 \scriptsize{$\pm$ 0.4}  & 31.9 \scriptsize{$\pm$ 1.0}      \\
        $F + C_{S,V}$ & +1.2\%   & \bf 84.4 \scriptsize{$\pm$ 0.2} & 88.4 \scriptsize{$\pm$ 1.2} & \bf 71.3 \scriptsize{$\pm$ 1.2}  & 67.4 \scriptsize{$\pm$ 0.9} & 69.3 \scriptsize{$\pm$ 3.7} & \bf 62.5 \scriptsize{$\pm$ 0.7}  & \bf 64.5 \scriptsize{$\pm$ 0.9}  & \bf 32.1 \scriptsize{$\pm$ 1.0}      \\
        
        \cdashlinelr{1-10}
        
        $F + C_{S,V}$ & +61\%  & 84.0 \scriptsize{$\pm$ 0.4} & 88.4 \scriptsize{$\pm$ 2.6} & 68.7 \scriptsize{$\pm$ 1.2}  & 66.2 \scriptsize{$\pm$ 0.8} & 68.3 \scriptsize{$\pm$ 2.8} & 62.1 \scriptsize{$\pm$ 0.3}  & 63.9 \scriptsize{$\pm$ 0.2}  & 31.7 \scriptsize{$\pm$ 0.9}      \\
        $F + C_{S}$ & +100\%    & 80.9 \scriptsize{$\pm$ 0.6} & 84.9 \scriptsize{$\pm$ 1.9} & 61.9 \scriptsize{$\pm$ 4.2}  & 63.5 \scriptsize{$\pm$ 0.5} & 61.7 \scriptsize{$\pm$ 3.8} & 59.6 \scriptsize{$\pm$ 0.6}  & 61.2 \scriptsize{$\pm$ 0.9}  & 30.7 \scriptsize{$\pm$ 0.7}      \\


        \cdashlinelr{1-10}
        \multicolumn{3}{l}{\textit{With agreement regularization:}} \\
        $F\ \&\ C_{S, V}$ & 61\%    & 83.0 \scriptsize{$\pm$ 0.3} & 89.2 \scriptsize{$\pm$ 1.1} & 65.8 \scriptsize{$\pm$ 1.1}  & 58.3 \scriptsize{$\pm$ 0.6} & \bf 71.2 \scriptsize{$\pm$ 1.9} & 61.1 \scriptsize{$\pm$ 0.4}  & 63.3 \scriptsize{$\pm$ 0.3}  & 31.4 \scriptsize{$\pm$ 0.8}      \\
        $F\ \&\ C_{S}$ & 100\%       & 80.7 \scriptsize{$\pm$ 0.4} & 82.4 \scriptsize{$\pm$ 3.5} & 59.1 \scriptsize{$\pm$ 2.2}  & 56.9 \scriptsize{$\pm$ 0.8} & 65.2 \scriptsize{$\pm$ 1.9} & 58.4 \scriptsize{$\pm$ 0.3}  & 60.6 \scriptsize{$\pm$ 0.7}  & 30.5 \scriptsize{$\pm$ 0.8}      \\
        
        
        \bottomrule
    \end{tabular}
    \caption{SPECTRA accuracy on in-domain datasets trained on SNLI factual examples ($F$), and with human-crafted counterfactual data augmentation ($F + C_H$). Counterfactual augmentation with synthetic examples are marked with ($C_S$), which we additionally post-processed to drop invalid examples ($C_{S,V}$).}
    \label{tab:results_rationalizers_in_domain_snli}
\end{table*}





\begin{table*}[t]
    \small
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l@{}rcccccccc}
        \toprule
        \textbf{Setup} & \bf Data Size & \cellcolor{cid}{SNLI} & \cellcolor{cid}{HNLI-e} & \cellcolor{cid}{HNLI-h} & \cellcolor{ccon}{rSNLI} & \cellcolor{ccon}{break} & \cellcolor{cood}{MNLI-m} & \cellcolor{cood}{MNLI-mm} & \cellcolor{cood}{ANLI} \\

        \midrule
        
        $F$         & 100\%      & 86.6 \scriptsize{$\pm$ 0.2} & 88.6 \scriptsize{$\pm$ 1.0} & 73.7 \scriptsize{$\pm$ 0.2} & 71.1 \scriptsize{$\pm$ 0.8} & 69.5 \scriptsize{$\pm$ 1.5} & 64.6 \scriptsize{$\pm$ 1.1} & 65.9 \scriptsize{$\pm$ 0.9} & 32.6 \scriptsize{$\pm$ 0.7} \\
        
        $F + C_H$   & +1.2\%     & 86.6 \scriptsize{$\pm$ 0.3} & 89.8 \scriptsize{$\pm$ 1.2} & 74.9 \scriptsize{$\pm$ 1.1} & \bf 72.4 \scriptsize{$\pm$ 0.3} & 70.1 \scriptsize{$\pm$ 1.9} & 64.2 \scriptsize{$\pm$ 0.9} & 65.8 \scriptsize{$\pm$ 0.9} & 31.8 \scriptsize{$\pm$ 0.4} \\


        \cdashlinelr{1-10}
        
        $F + C_{S,V}$ & +0.25\%  & \bf 86.9 \scriptsize{$\pm$ 0.2} & 87.3 \scriptsize{$\pm$ 3.7} & 75.2 \scriptsize{$\pm$ 1.1} & 71.4 \scriptsize{$\pm$ 0.8} & 68.6 \scriptsize{$\pm$ 1.7} & 64.4 \scriptsize{$\pm$ 0.7} & 65.7 \scriptsize{$\pm$ 0.4} & 32.2 \scriptsize{$\pm$ 1.5}  \\
        
        $F + C_{S,V}$ & +0.5\%   & 86.7 \scriptsize{$\pm$ 0.1} & 87.7 \scriptsize{$\pm$ 3.3} & 74.1 \scriptsize{$\pm$ 1.7} & 71.5 \scriptsize{$\pm$ 0.3} & 69.6 \scriptsize{$\pm$ 1.7} & \bf 64.8 \scriptsize{$\pm$ 0.7} & 66.0 \scriptsize{$\pm$ 0.9} & 31.8 \scriptsize{$\pm$ 0.8} \\
        
        $F + C_{S,V}$ & +1.0\%   & 86.7 \scriptsize{$\pm$ 0.1} & 87.4 \scriptsize{$\pm$ 3.1} & 75.3 \scriptsize{$\pm$ 2.3} & 72.1 \scriptsize{$\pm$ 0.6} & 68.3 \scriptsize{$\pm$ 1.3} & 64.3 \scriptsize{$\pm$ 0.6} & 65.9 \scriptsize{$\pm$ 0.5} & 31.9 \scriptsize{$\pm$ 0.7}  \\
        
        $F + C_{S,V}$ & +1.2\%   & \bf  86.9 \scriptsize{$\pm$ 0.3} & 88.4 \scriptsize{$\pm$ 0.9} & 75.5 \scriptsize{$\pm$ 1.5} & 71.4 \scriptsize{$\pm$ 1.2} & 69.8 \scriptsize{$\pm$ 2.2} & 64.0 \scriptsize{$\pm$ 1.1} & 65.3 \scriptsize{$\pm$ 1.0} & 33.0 \scriptsize{$\pm$ 1.2}  \\

        \cdashlinelr{1-10}
        
        $F + C_{S,V}$ & +42\%   & 86.5 \scriptsize{$\pm$ 0.3} & 88.2 \scriptsize{$\pm$ 1.6} & \bf 75.8 \scriptsize{$\pm$ 1.2} & 71.8 \scriptsize{$\pm$ 1.0} & 69.1 \scriptsize{$\pm$ 2.0} & 64.4 \scriptsize{$\pm$ 0.3} & 65.9 \scriptsize{$\pm$ 0.4} & 32.2 \scriptsize{$\pm$ 0.2} \\
        
        $F + C_{S}$   & +100\%  & 86.6 \scriptsize{$\pm$ 0.3} & 89.0 \scriptsize{$\pm$ 2.6} & 74.7 \scriptsize{$\pm$ 1.1} & 71.6 \scriptsize{$\pm$ 0.8} & \bf 71.2 \scriptsize{$\pm$ 1.4} & 64.5 \scriptsize{$\pm$ 0.4} & \bf 66.4 \scriptsize{$\pm$ 0.6} & 32.2 \scriptsize{$\pm$ 1.0} \\

        \cdashlinelr{1-10}
        \multicolumn{3}{l}{\textit{With agreement regularization:}} \\
        $F\ \&\ C_{S, V}$ & 42\%    & 86.8 \scriptsize{$\pm$ 0.1} & 90.4 \scriptsize{$\pm$ 1.3} & 75.3 \scriptsize{$\pm$ 0.8} & 66.8 \scriptsize{$\pm$ 0.7} & 68.2 \scriptsize{$\pm$ 2.1} & 64.6 \scriptsize{$\pm$ 0.7} & 66.1 \scriptsize{$\pm$ 0.6} & \bf 32.8 \scriptsize{$\pm$ 0.6}  \\
        
        $F\ \&\ C_{S}$    & 100\%   & 86.6 \scriptsize{$\pm$ 0.1} & \bf 90.6 \scriptsize{$\pm$ 1.3} & 75.5 \scriptsize{$\pm$ 1.3} & 67.0 \scriptsize{$\pm$ 1.3} & 69.9 \scriptsize{$\pm$ 1.7} & 64.2 \scriptsize{$\pm$ 1.1} & 66.0 \scriptsize{$\pm$ 0.7} & 32.5 \scriptsize{$\pm$ 0.5}\\
        
        \bottomrule
    \end{tabular}
    \caption{SPECTRA accuracy on in-domain datasets trained on SNLI factual examples ($F$), and with human-crafted counterfactual data augmentation ($F + C_H$). Counterfactual augmentation with synthetic examples are marked with ($C_S$), which we additionally post-processed to drop invalid examples ($C_{S,V}$).}
    \label{tab:results_rationalizers_in_domain_snli_hyp}
\end{table*}



\begin{table*}[!htb]
    \small
    \centering
    \begin{tabular}{l c@{\tquad}c@{\tquad}c}
        \toprule
        \bf Setup & \bf Plausibility & \bf F. sim. & \bf C. sim. \\
        \midrule
        $F$                       & 0.7735 \scriptsize{$\pm$ 0.00} & 59.26 \scriptsize{$\pm$ 0.41} & 70.01 \scriptsize{$\pm$ 0.44} \\
        $F + C_H$                 & 0.7736 \scriptsize{$\pm$ 0.01} & 59.51 \scriptsize{$\pm$ 0.86} & 69.90 \scriptsize{$\pm$ 0.57} \\
        $F + C_S$                 & 0.7779 \scriptsize{$\pm$ 0.00} & \bf 59.54 \scriptsize{$\pm$ 0.08} & \bf 70.76 \scriptsize{$\pm$ 0.54} \\
        \cdashlinelr{1-4}
        \multicolumn{3}{l}{\textit{With agreement regularization:}} \\
        $F\ \&\ C_S$              & \bf 0.7808 \scriptsize{$\pm$ 0.00} & 59.31 \scriptsize{$\pm$ 0.20} & 70.69 \scriptsize{$\pm$ 0.29} \\
        
        \bottomrule
    \end{tabular}
    \caption{Interpretability analysis. Plausibility represents matching with human rationales in terms of AUC, whereas F. sim. and C. sim. represent forward and counterfactual simulability, respectively.}
\end{table*}

